Faithful Explanations for Deep Graph Models

This paper studies faithful explanations for Graph Neural Networks (GNNs). First, we provide a new and general method for formally characterizing the faithfulness of explanations for GNNs. It applies to existing explanation methods, including feature attributions and subgraph explanations. Second, our analytical and empirical results demonstrate that feature attribution methods cannot capture the nonlinear effect of edge features, while existing subgraph explanation methods are not faithful. Third, we introduce \emph{k-hop Explanation with a Convolutional Core} (KEC), a new explanation method that provably maximizes faithfulness to the original GNN by leveraging information about the graph structure in its adjacency matrix and its \emph{k-th} power. Lastly, our empirical results over both synthetic and real-world datasets for classification and anomaly detection tasks with GNNs demonstrate the effectiveness of our approach.

==> Figure_khop_model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=80mm]{images/squared_A.png}
    \caption{The square of an adjacency matrix}
    \label{fig:square_of_a}
\end{figure}

==> Figure_non_linearity.tex <==
\begin{figure}
\centering     %%% not \center

\subcaptionbox{\label{fig:lineari-p-X}}{\includegraphics[width=35mm]{images/linear.png}}
\hfill
\subcaptionbox{\label{fig:lineari-p-A}}{\includegraphics[width=35mm]{images/nonlinear.png}}

\caption{\subref{fig:lineari-p-X} The input space of $X$ when $A$ is fixed. \subref{fig:lineari-p-A} The input space of $A$ when $X$ is fixed. Facets of activation polytopes are in black. \carlee{Define $F$ and what an activation region is in the caption.}}

\end{figure}


==> Figure_soft_tree.tex <==
\begin{figure}
    \centering
    \includegraphics[width=60mm]{images/soft_tree.png}
    \caption{An example soft tree (depth=2). The leaf nodes are colored in green and others are in blue. The output of this tree for an input $x$ is shown on the right side as $\text{softmax}((1-\sigma_0)\sigma_1)\cdot w^\top x$ where the softmax is taken over all leaves.}
    \label{fig:soft-tree-example}
\end{figure}

==> Figure_sparsity.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\columnwidth]{images/sparsity.png}
    \caption{The performance of different explanations on Cora (measured with general unfaithfulness and the AUC score of edge sparsity) against the performance of the GNN model on the test nodes (measured with the classification accuracy score).}
    \label{fig:sprasity}
\end{figure}

==> Figure_visualization.tex <==

\begin{figure*}[t]
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{input.png}\\
        \subcaption{Input Computation Graph}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/SoftGNNExplainer.png}\\
        \subcaption{GNN Explainer}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{acmsmall-mouse.pdf}\\
        \subcaption{PG Explainer}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/KEC.png}\\
        \subcaption{KEC}
    \end{minipage}%
    \\
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{acmsmall-mouse.pdf}\\
        \subcaption{Linear}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/Saliency.png}\\
        \subcaption{Saliency Map}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/ZeroIG.png}\\
        \subcaption{Integrated Gradient (zero)}
    \end{minipage}%
    \begin{minipage}[b]{0.25\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{images/RandomIG.png}\\
        \subcaption{Integrated Gradient (random)}
    \end{minipage}%
\caption{Visualization of graph explanations for Cora using a GNN that achieves an accuracy of 80.4\% on the test split. The quantity of interest is the output score of the predicted class for Node 9 (in black). The computational graph is shown in (a) and explanations are visualized from (b) to (h). The node importance is the sum of feature importance scores and less transparent nodes have higher positive contributions. The sign of the edge importance is colored with red (positive), blue (negative) and black (zeros) and the thickness corresponds to the magnitude. All scores are normalized to $[-1, 1]$ for the purpose of visualization.}
\end{figure*}

==> Tabel_dataset_statistics.tex <==
\begin{table}[h]
    \small
    \centering
    \begin{tabular}{l|cccc}
    \toprule\toprule
   Dataset& Nodes &Edges & Features &Classes \\
    \midrule
          BA-Shapes & 700 & 2,055 & - &4 \\
          Cora & 2,708 & 5,429 & 1,433 &7 \\
          Citeseer & 3,327 & 4,732 & 3,703 &6 \\
     \bottomrule
    \end{tabular}
    \caption{Statistics of Datasets.}
    \label{tab:dataset_statistics}
\end{table}



==> Table_timing.tex <==
% \begin{table}[t]
%   \small
%   \centering
%   \begin{tabular}{l|ccc}
   
%   \toprule\toprule
%   & \text{BA-shapes} & \text{Cora} & \text{Citeseer} \\ 
%   \midrule
%   GNNExpl (100 epochs) & 0.70 & 0.50	& 0.53\\
%   PGExpl & 0.62&	0.45	&0.47\\
%   SM & 8.03 $\times 10^{-3}$	&1.36 $\times 10^{-2}$	&6.91 $\times 10^{-2}$\\
%   IG (50 samples) & 2.34 $\times 10^{-2}$	&0.45	&1.45\\
%   Linear (200 samples) & 1.01 $\times 10^{-3}$ 	&1.20 $\times 10^{-2}$	&3.54 $\times 10^{-2}$\\
%   Linear (1500 samples)& 1.17 $\times 10^{-3}$	&1.23 $\times 10^{-2}$	&3.58 $\times 10^{-2}$\\
%   KEC (200 samples) & 3.71 $\times 10^{-2}$	& 3.11 $\times 10^{-2}$	& 5.77 $\times 10^{-2}$\\
%   KEC (1500 samples) & 3.76 $\times 10^{-2}$	&3.13 $\times 10^{-2}$ &	5.78 $\times 10^{-2}$\\
%   \bottomrule
   
%   \end{tabular} 
%   \caption{Efficiency of different methods measured on one Titan RTX. We include the training time for GNNExpl and PGExpl. } \label{tab:efficiency}
% \end{table}


\begin{table}[t]
  \small
  \centering
  \begin{tabular}{l|ccc}
  \toprule\toprule
  & \text{BA-shapes} & \text{Cora} & \text{Citeseer} \\ 
  \# of GCN layers& 3 & 2& 2 \\ 
  \midrule
  GNNExpl (100 epochs) & 0.70 & 0.50	& 0.53\\
  PGExpl (30 epochs) & 0.62&	0.45	&0.47\\
  SM & 0.01	&0.01	&0.07\\
  IG (50 samples) & 0.02	&0.45	&1.45\\
  Linear (200 samples) & 1.01 $\times 10^{-3}$ 	&0.01	&0.04\\
  Linear (1500 samples)& 1.17 $\times 10^{-3}$	&0.01	&0.04\\
  KEC (200 samples) & 0.04	&0.03	&0.06\\
  KEC (1500 samples) & 0.04	&0.03	&0.06\\
  \bottomrule
  \end{tabular} 
  \caption{Per node running time (unit: second) measured on one Tesla T4. We include the training time for GNNExpl and PGExpl. Results are averaged over 100 nodes. } \label{tab:efficiency}
\end{table}



% \begin{table}[t]
%   \small
%   \centering
%   \begin{tabular}{l|ccc}
%   \toprule\toprule
%   & BA-shapes & Cora & Citeseer \\ 
%   \midrule
%   GNNExpl (100 epochs) & 42.2023 & 49.74 & 52.68\\
%   PGExpl & 37.2535 & 45.30 & 46.81\\
%   SM & 0.482058 & 1.36 & 6.91\\
%   IG (50 samples) & 1.40673 & 45.14 & 144.78\\
%   Linear (200 samples) & 0.0608292 & 1.20 & 3.54 \\
%   Linear (1500 samples)& 0.0704463 & 1.23 & 3.58\\
%   KEC (200 samples) & 2.22464 & 3.11 & 5.77\\
%   KEC (1500 samples) & 2.25747 & 3.13 & 5.78\\
%   \bottomrule
%   \end{tabular} 
%   \caption{Efficiency of different methods measured on one Titan RTX. We include the training time for GNNExpl and PGExpl. } \label{tab:efficiency}
% \end{table}

% \begin{table}[t]
%   \small
%   \centering
%   \begin{tabular}{l|ccc}
%   \toprule\toprule
%   & BA-shapes & Cora & Citeseer \\ 
%   \midrule
%   GNNExpl (100 epochs) & 67.8581 & 49.74 & 52.68\\
%   PGExpl & 51.3333 & 45.30 & 46.81\\
%   SM & 0.761057 & 1.36 & 6.91\\
%   IG (50 samples) & 2.01312 & 45.14 & 144.78\\
%   Linear (200 samples) & 0.0936086 & 1.20 & 3.54 \\
%   Linear (1500 samples)& 0.121773 & 1.23 & 3.58\\
%   KEC (200 samples) & 3.49638 & 3.11 & 5.77\\
%   KEC (1500 samples) & 3.40048 & 3.13 & 5.78\\
%   \bottomrule
%   \end{tabular} 
%   \caption{Efficiency of different methods measured on one Titan RTX. We include the training time for GNNExpl and PGExpl. } \label{tab:efficiency}
% \end{table}


% \begin{table}[t]
%   \small
%   \centering
%   \begin{tabular}{l|ccc}
%   \toprule\toprule
%   & BA-shapes & Cora & Citeseer \\ 
%   \midrule
%   GNNExpl (100 epochs) & 69.4192 & 49.7379 & 52.6764\\
%   PGExpl & 107.845 & 45.2958 & 46.8075\\
%   SM & 0.841897 & 1.36141 & 6.91425\\
%   IG (50 samples) & 2.67187 & 45.1419 & 144.784\\
%   Linear (200 samples) & 0.104733 & 1.2059 & 3.54103 \\
%   Linear (1500 samples)& 0.143279 & 1.23416 & 3.57546\\
%   KEC (200 samples) & 3.51431 & 3.11259 & 5.77003\\
%   KEC (1500 samples) & 3.53309 & 3.13487 & 5.78041\\
%   \bottomrule
%   \end{tabular} 
%   \caption{Efficiency of different methods measured on one Titan RTX. We include the training time for GNNExpl and PGExpl. } \label{tab:efficiency}
% \end{table}

==> section_checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
	  \answerYes{}
  \item Did you describe the limitations of your work?
	  \answerYes{See Approximation Error in Section~\ref{sec:evaluations} and Explaining Graph Classifications in Section~\ref{sec:related-work}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
	  \answerYes{}
        \item Did you include complete proofs of all theoretical results?
		\answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include it in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
	  \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{See}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
	  \answerYes{}
  \item Did you mention the license of the assets?
	  \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Yes}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
	  \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


